Cognacy Queries over Dependence Graphs for Transparent Visualisations

Charts, figures, and text derived from data play an important role in decision making, from data-driven policy development to day-to-day choices informed by online articles. Making sense of, or fact-checking, outputs means understanding how they relate to the underlying data. Even for domain experts with access to the source code and data sets, this poses a significant challenge. In this paper we introduce a new program analysis framework which supports interactive exploration of fine-grained I/O relationships directly through computed outputs, making use of dynamic dependence graphs. Our main contribution is a novel notion in data provenance which we call related inputs, a relation of mutual relevance or "cognacy" which arises between inputs when they contribute to common features of the output. Queries of this form allow readers to ask questions like "What outputs use this data element, and what other data elements are used along with it?". We show how Jonsson and Tarski's concept of conjugate operators on Boolean algebras appropriately characterises the notion of cognacy in a dependence graph, and give a procedure for computing related inputs over such a graph.

==> fig/basic-elements.tex <==
\begin{figure}[H]
\small
\begin{tabularx}{\textwidth}{rll}
   $n, m \in$
   &
   $\Int$
   &
   integer
   \\
   $i, j \in$
   &
   $\set{n \in \Int \mid n \numgeq 1}$
   &
   positive integer
   \\
   $z \in$
   &
   $\Str$
   &
   finite sequence of characters
   \\
   $x, y, f, \oplus \in$
   &
   $\Var$
   &
   variable
   \\
   $c \in$
   &
   $\Ctr$
   &
   constructor name
   \\
   $D \in$
   &
   $\DataType$
   &
   datatype name
\end{tabularx}
\caption{Basic elements}
\label{fig:basic-elements}
\end{figure}


==> fig/core/typing.tex <==
\begin{figure}
   \small{\flushleft \shadebox{$\Gamma \vdash e: A$}%
   \hfill \textbfit{$e$ has type $A$ under $\Gamma$}}
   \begin{smathpar}
   \inferrule*[right={$x : A \in \Gamma$}]
   {
      \strut
   }
   {
      \Gamma \vdash \exVar{x}: A
   }
   %
   \and
   %
   \inferrule*
   {
      \strut
   }
   {
      \Gamma \vdash \exInt{n}: \tyInt
   }
   %
   \and
   %
   \inferrule*[
      right={$\datatype{c} = \tyForeign{\seq{A}}{D}$}
   ]
   {
      \Gamma \vdash \seq{e: A}
   }
   {
      \Gamma \vdash \exConstr{c}{\seq{e}}: D
   }
   %
   \and
   %
   \inferrule*
   {
      \Gamma \vdash e_i: \tyStr
      \\
      \Gamma \vdash e'_i: A
      \quad
      (\forall i \numleq \length{\seq{e}})
   }
   {
      \Gamma \vdash \exDict{\seq{\bind{e}{e}}'}: \tyDict{A}
   }
   %
   \and
   %
   \inferrule*
   {
      \Gamma \vdash \seq{e: A}
   }
   {
      \Gamma \vdash \exRec{\seq{\bind{x}{e}}}: \tyRec{\seq{\bind{x}{A}}}
   }
   %
   \and
   %
   \inferrule*[
      right={$i \numleq \length{\seq{x}}$}
   ]
   {
      \Gamma \vdash e: \tyRec{\seq{\bind{x}{A}}}
   }
   {
      \Gamma \vdash \exRecProj{e}{x_i}: A_i
   }
   %
   \and
   %
   \inferrule*
   {
      \Gamma \vdash \sigma : \elimTy{A}{B}
   }
   {
      \Gamma \vdash \exFun{\sigma} : \tyFun{A}{B}
   }
   %
   \and
   %
   \inferrule*[
      right={$f: \tyForeign{\seq{A}}{B} \in \Phi$}
   ]
   {
      \Gamma \vdash \seq{e: A}
   }
   {
      \Gamma \vdash f(\seq{e}): B
   }
   %
   \and
   %
   \inferrule*
   {
      \Gamma \vdash e: \tyFun{A}{B}
      \\
      \Gamma \vdash e': A
   }
   {
      \Gamma \vdash \exApp{e}{e'}: B
   }
   %
   \and
   %
   \inferrule*
   {
      \Gamma \vdash \rho: \Delta
      \\
      \Gamma \concat \Delta \vdash e: A
   }
   {
      \Gamma \vdash \exLetRec{\rho}{e}: A
   }
   \end{smathpar}
   \\[2mm]
   {\small \flushleft \shadebox{$\Gamma \vdash \sigma: \elimTy{A}{K}$}%
   \hfill \textbfit{$\sigma$ has type $\elimTy{A}{K}$ under $\Gamma$}}
   \begin{smathpar}
   \inferrule*
   {
      \Gamma \cons \bind{x}{A} \vdash \kappa: K
   }
   {
      \Gamma \vdash (\elimVar{x}{\kappa}): \elimTy{A}{K}
   }
   %
   \and
   %
   \inferrule*
   {
      (\datatype{c_i} = \tyForeign{\seq{A}_i}{D} \in
       \implies
       \Gamma \vdash \kappa_i: \elimTy{\seq{A}_i}{K})
      \quad
      (\forall i \numleq \length{\seq{c}})
   }
   {
      \Gamma \vdash \{\seq{\elimBind{c}{\kappa}}\}: \elimTy{D}{K}
   }
   %
   \and
   %
   \inferrule*
   {
      \Gamma \vdash \kappa: K
   }
   {
      \Gamma
      \vdash
      \elimRecord{}{\kappa}: \elimTy{\tyRecEmpty}{K}
   }
   %
   \and
   %
   \inferrule*
   {
      \Gamma \vdash \elimRecord{\seq{x}}{\sigma}: \elimTy{\tyRec{\seq{\bind{x}{A}}}}{\elimTy{B}{K}}
   }
   {
      \Gamma
      \vdash
      \elimRecord{\seq{x} \cons y}{\sigma}: \elimTy{\tyRec{\seq{\bind{x}{A}} \cons \bind{y}{B}}}{K}
   }
   \end{smathpar}
   \\[2mm]
   {\small \flushleft \shadebox{$\vdash v: A$}%
   \hfill \textbfit{$v$ has type $A$}}
   \begin{smathpar}
   \inferrule*
   {
      \strut
   }
   {
      \vdash \exInt{n}: \tyInt
   }
   %
   \and
   %
   \inferrule*
   {
      \vdash \seq{v: A}
   }
   {
      \vdash \exRec{\seq{\bind{x}{v}}}: \tyRec{\seq{\bind{x}{A}}}
   }
   %
   \and
   %
   \inferrule*
   {
      \vdash \gamma: \Gamma
      \\
      \Gamma \vdash \rho: \Delta
      \\
      \Gamma \concat \Delta \vdash \sigma: \elimTy{A}{B}
   }
   {
      \vdash \exClosure{\gamma}{\rho}{\sigma}: \tyFun{A}{B}
   }
   %
   \and
   %
   \inferrule*[
      right={$\datatype{c} = \tyForeign{\seq{A}}{D}$}
   ]
   {
      \Gamma \vdash \seq{v: A}
   }
   {
      \Gamma \vdash \exConstr{c}{\seq{v}}: \tyData{D}
   }
   \end{smathpar}
   \\[2mm]
   \begin{minipage}[t]{0.4\textwidth}%
   {\small \flushleft \shadebox{$\vdash \gamma: \Gamma$}%
   \hfill \textbfit{$\gamma$ has type $\Gamma$}}
   \begin{smathpar}
   \inferrule*
   {
      \vdash \seq{v: A}
   }
   {
      \vdash \seq{\bind{x}{v}}: \seq{\bind{x}{A}}
   }
   \end{smathpar}
   \end{minipage}%
   \hspace{5mm}%
   \begin{minipage}[t]{0.5\textwidth}%
   {\small \flushleft \shadebox{$\Gamma \vdash \rho: \Delta$}%
   \hfill \textbfit{$\rho$ has type $\Delta$ under $\Gamma$}}
   \begin{smathpar}
      \inferrule*[right={
         \textnormal{$\Delta = \seq{\bind{x}{\tyFun{A}{B}}}$}
      }]
      {
         \Gamma \concat \Delta \vdash \seq{\sigma: \elimTy{A}{B}}
      }
      {
         \Gamma \vdash \seq{\bind{x}{\sigma}}: \Delta
      }
   \end{smathpar}
   \end{minipage}
   \caption{Typing rules for core language}
   \label{fig:core-language:typing}
\end{figure}


==> fig/example/obsolete/surface-examples.tex <==
\begin{figure}
   \begin{subfigure}{0.44\textwidth}
      \tiny
      \lstinputlisting[language=Fluid]{fig/example/surface/filter.fld}
      \caption{Piecewise functions}
      \label{fig:core:surface-examples:functions}
   \end{subfigure}
   \begin{subfigure}{0.44\textwidth}
      \tiny
      \lstinputlisting[language=Fluid]{fig/example/surface/matrix.fld}
      \caption{Matrix syntax}
      \label{fig:core:surface-examples:matrix}
   \end{subfigure}
   \vfill
   \begin{subfigure}{0.44\textwidth}
      \tiny
      \lstinputlisting[language=Fluid]{fig/example/surface/list-comp.fld}
      \caption{List comprehensions}
      \label{fig:core:surface-examples:listcomps}
   \end{subfigure}
   \begin{subfigure}{0.44\textwidth}
      \tiny
      \lstinputlisting[language=Fluid]{fig/example/surface/dict_record.fld}
      \caption{Dictionaries and records}
      \label{fig:core:surface-examples:dicts}
   \end{subfigure}
   \caption{Some example programs in our surface language}
   \label{fig:core:surface-examples}
\end{figure}

==> fig/performance/all-benches.tex <==
\begin{table}
\caption{All test-cases and all benchmarks, TODO: needs formatting somehow}
\label{table:all-benches}
\begin{tabular}{lllllllllll}
\toprule
 & G-Bwd & G-BwdAll & G-BwdDlCmp & G-BwdDlFwdOp & G-Eval & G-Fwd & G-FwdDlBwdOp & G-FwdDlCmp & Graph-Nodes & Naive-Fwd & T-Bwd & T-Eval & T-Fwd \\
Test-Name &  &  &  &  &  &  &  &  &  &  &  &  &  \\
\midrule
desugar/list-comp-1 & (0.5 : 0.07071069497739416 : Nil) & (9.099999994039536 : 0.8485281500679115 : Nil) & (0.5999999940395355 : 0.2121320217119097 : Nil) & (33.54999998211861 : 5.409366880291773 : Nil) & (0.9000000059604645 : 0.2121320217119097 : Nil) & (134.0 : 0.0 : Nil) & (11.299999982118607 : 0.7778174550905174 : Nil) & (17.450000017881393 : 3.2880465367321308 : Nil) & (16.950000017881393 : 3.4294678845400703 : Nil) & (12.400000005960464 : 1.9798989746782785 : Nil) \\
desugar/list-comp-2 & (0.15000000596046448 : 0.0 : Nil) & (23.899999976158142 : 0.21213204278533396 : Nil) & (0.2499999701976776 : 0.03535532641527282 : Nil) & (74.60000002384186 : 1.6970562579889745 : Nil) & (0.4000000059604645 : 0.0 : Nil) & (417.5 : 0.0 : Nil) & (28.5 : 0.9192388239718814 : Nil) & (28.749999970197678 : 1.6617009315737017 : Nil) & (31.0 : 1.1313708667572153 : Nil) & (27.5 : 0.9192388239718814 : Nil) \\
desugar/list-comp-3 & (0.29999998211860657 : 2.1073424255447014e-8 : Nil) & (6.5999999940395355 : 2.1073424255447014e-8 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (18.349999994039536 : 0.6010407597938805 : Nil) & (0.9000000059604645 : 0.14142136888136406 : Nil) & (130.0 : 0.0 : Nil) & (5.999999970197678 : 0.14142136888136406 : Nil) & (7.249999970197678 : 0.10606602139266698 : Nil) & (6.8499999940395355 : 0.10606602139266698 : Nil) & (6.799999982118607 : 0.0707106739039699 : Nil) \\
desugar/list-comp-4 & (0.3499999940395355 : 0.10606602139266698 : Nil) & (2.550000011920929 : 0.10606600031924272 : Nil) & (0.0 : 0.0 : Nil) & (6.649999976158142 : 0.10606600031924272 : Nil) & (0.5 : 0.07071065283054564 : Nil) & (55.5 : 0.0 : Nil) & (2.300000011920929 : 0.1414213478079398 : Nil) & (2.3000000417232513 : 0.0707106739039699 : Nil) & (2.4000000059604645 : 0.0707106739039699 : Nil) & (2.5 : 0.2828426956158796 : Nil) \\
desugar/list-comp-5 & (0.09999999403953552 : 0.0 : Nil) & (1.9000000059604645 : 0.14142136888136406 : Nil) & (0.20000001788139343 : 0.0707106739039699 : Nil) & (4.350000023841858 : 0.03535534748869708 : Nil) & (0.19999998807907104 : 0.0 : Nil) & (40.0 : 0.0 : Nil) & (1.6500000059604645 : 0.17677671637006112 : Nil) & (1.3499999642372131 : 0.03535534748869708 : Nil) & (2.0999999940395355 : 2.1073424255447014e-8 : Nil) & (1.949999988079071 : 0.31819804310457667 : Nil) \\
desugar/list-comp-6 & (0.0 : 0.0 : Nil) & (0.04999998211860657 : 0.0 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.3499999940395355 : 0.10606602139266698 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (4.0 : 0.0 : Nil) & (0.09999999403953552 : 0.0707106739039699 : Nil) & (0.20000001788139343 : 0.0707106739039699 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.0 : 0.0 : Nil) \\
desugar/list-comp-7 & (0.20000001788139343 : 2.1073424255447014e-8 : Nil) & (2.5 : 0.07071069497739416 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (3.900000035762787 : 0.8485281289944873 : Nil) & (0.44999998807907104 : 0.10606600031924272 : Nil) & (46.5 : 0.0 : Nil) & (1.550000011920929 : 0.03535534748869708 : Nil) & (1.350000023841858 : 0.03535534748869708 : Nil) & (1.5499999821186066 : 0.6010407597938805 : Nil) & (1.9000000059604645 : 0.14142136888136406 : Nil) \\
desugar/list-enum & (0.04999998211860657 : 0.03535532641527282 : Nil) & (1.550000011920929 : 0.03535534748869708 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (3.150000035762787 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (31.5 : 0.0 : Nil) & (0.949999988079071 : 0.03535534748869708 : Nil) & (0.44999998807907104 : 0.0 : Nil) & (0.8499999642372131 : 0.17677669529663687 : Nil) & (0.5 : 0.0 : Nil) \\
arithmetic & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.3500000238418579 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 0.0707106739039699 : Nil) & (1.050000011920929 : 0.10606600031924272 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (11.5 : 0.0 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (0.29999998211860657 : 0.0707106739039699 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) \\
array & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.75 : 0.03535534748869708 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (2.8499999940395355 : 0.9545941503871542 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (20.5 : 0.0 : Nil) & (0.3999999761581421 : 0.07071069497739416 : Nil) & (1.199999988079071 : 0.35355339059327373 : Nil) & (1.5 : 0.9192388239718814 : Nil) & (0.20000001788139343 : 0.0 : Nil) \\
compose & (0.050000011920928955 : 0.0 : Nil) & (0.6500000059604645 : 0.035355368562121334 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.7500000298023224 : 0.03535532641527282 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (6.5 : 0.0 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.6499999761581421 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (0.25 : 0.03535534748869708 : Nil) \\
dicts & (0.15000003576278687 : 0.03535534748869708 : Nil) & (1.949999988079071 : 0.17677669529663687 : Nil) & (0.20000001788139343 : 0.0707106739039699 : Nil) & (3.4500000178813934 : 0.6717514547712746 : Nil) & (0.45000001788139343 : 0.10606602139266698 : Nil) & (29.5 : 0.0 : Nil) & (0.19999998807907104 : 0.0 : Nil) & (1.75 : 0.03535534748869708 : Nil) & (1.0499999821186066 : 0.38890871700854657 : Nil) & (0.44999998807907104 : 0.03535534748869708 : Nil) \\
div-mod-quot-rem & (0.25 : 0.03535534748869708 : Nil) & (2.8499999940395355 : 0.0 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (7.5 : 0.1414213478079398 : Nil) & (1.649999976158142 : 0.03535534748869708 : Nil) & (75.0 : 0.0 : Nil) & (0.25 : 0.0 : Nil) & (0.6499999761581421 : 0.03535534748869708 : Nil) & (0.4000000059604645 : 0.0 : Nil) & (0.5999999940395355 : 2.1073424255447014e-8 : Nil) \\
factorial & (0.1499999761581421 : 0.03535534748869708 : Nil) & (2.850000023841858 : 0.17677669529663687 : Nil) & (0.09999999403953552 : 0.0707106739039699 : Nil) & (7.249999970197678 : 0.3181980641780009 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (48.5 : 0.0 : Nil) & (0.8499999940395355 : 0.0 : Nil) & (2.149999976158142 : 0.03535534748869708 : Nil) & (2.0000000298023224 : 0.14142136888136406 : Nil) & (2.0499999821186066 : 0.24748736920060677 : Nil) \\
filter & (0.09999999403953552 : 0.0 : Nil) & (1.0499999821186066 : 0.03535532641527282 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (3.1999999582767487 : 0.28284271668930383 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (24.0 : 0.0 : Nil) & (0.699999988079071 : 0.0 : Nil) & (1.0500000417232513 : 0.10606602139266698 : Nil) & (1.050000011920929 : 0.03535534748869708 : Nil) & (1.25 : 0.17677669529663687 : Nil) \\
first-class-constr & (0.15000003576278687 : 0.03535534748869708 : Nil) & (1.699999988079071 : 0.07071069497739416 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (3.350000023841858 : 0.31819804310457667 : Nil) & (0.19999998807907104 : 0.0 : Nil) & (33.0 : 0.0 : Nil) & (0.9500000178813934 : 0.03535532641527282 : Nil) & (1.0999999940395355 : 0.2121320217119097 : Nil) & (1.5999999940395355 : 0.0707106739039699 : Nil) & (1.350000023841858 : 0.17677669529663687 : Nil) \\
flatten & (0.15000003576278687 : 0.03535534748869708 : Nil) & (1.2999999821186066 : 0.0 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (5.649999976158142 : 0.31819804310457667 : Nil) & (0.25 : 0.0 : Nil) & (43.5 : 0.0 : Nil) & (1.9000000059604645 : 2.1073424255447014e-8 : Nil) & (1.7000000178813934 : 0.0707106739039699 : Nil) & (2.399999976158142 : 0.1414213478079398 : Nil) & (2.4000000059604645 : 0.14142136888136406 : Nil) \\
foldr-sumSquares & (0.050000011920928955 : 0.0 : Nil) & (0.6499999761581421 : 0.03535534748869708 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (1.7000000178813934 : 0.0707106739039699 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (28.5 : 0.0 : Nil) & (0.3499999940395355 : 0.03535532641527282 : Nil) & (0.25 : 0.0 : Nil) & (0.4000000059604645 : 0.0707106739039699 : Nil) & (0.5499999821186066 : 0.03535532641527282 : Nil) \\
include-input-into-output & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.0 : 0.0 : Nil) & (0.0 : 0.0 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.0 : 0.0 : Nil) & (1.5 : 0.0 : Nil) & (0.0 : 0.0 : Nil) & (0.0 : 0.0 : Nil) & (0.0 : 0.0 : Nil) & (0.0 : 0.0 : Nil) \\
lexicalScoping & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.2500000298023224 : 0.10606602139266698 : Nil) & (0.0 : 0.0 : Nil) & (0.3500000238418579 : 0.03535534748869708 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (7.0 : 0.0 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (0.19999998807907104 : 0.07071069497739416 : Nil) & (0.09999999403953552 : 0.0 : Nil) \\
length & (0.0 : 0.0 : Nil) & (0.2500000298023224 : 0.03535532641527282 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.5499999821186066 : 0.10606602139266698 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (12.0 : 0.0 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.20000001788139343 : 2.1073424255447014e-8 : Nil) \\
lookup & (0.1499999761581421 : 0.03535534748869708 : Nil) & (1.600000023841858 : 0.07071069497739416 : Nil) & (0.0 : 0.0 : Nil) & (2.7000000178813934 : 0.0707106739039699 : Nil) & (0.45000001788139343 : 0.03535532641527282 : Nil) & (48.0 : 0.0 : Nil) & (0.5499999821186066 : 0.03535532641527282 : Nil) & (0.6499999761581421 : 0.03535534748869708 : Nil) & (0.75 : 0.10606600031924272 : Nil) & (0.75 : 0.03535534748869708 : Nil) \\
map & (0.0 : 0.0 : Nil) & (0.3499999940395355 : 0.0 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (1.6500000059604645 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (34.5 : 0.0 : Nil) & (0.19999998807907104 : 0.0 : Nil) & (0.5999999940395355 : 2.1073424255447014e-8 : Nil) & (0.44999998807907104 : 0.03535534748869708 : Nil) & (0.7499999701976776 : 0.03535532641527282 : Nil) \\
mergeSort & (0.04999998211860657 : 0.0 : Nil) & (1.0 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (6.0999999940395355 : 0.14142136888136406 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (80.0 : 0.0 : Nil) & (2.7000000178813934 : 0.0707106739039699 : Nil) & (1.7500000298023224 : 0.10606602139266698 : Nil) & (2.7999999821186066 : 0.14142136888136406 : Nil) & (2.8499999940395355 : 0.03535532641527282 : Nil) \\
normalise & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.4000000059604645 : 0.0707106739039699 : Nil) & (0.0 : 0.0 : Nil) & (0.4000000059604645 : 0.0707106739039699 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (14.0 : 0.0 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.1499999761581421 : 0.0 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (0.050000011920928955 : 0.0 : Nil) \\
nub & (0.050000011920928955 : 0.03535534748869708 : Nil) & (1.6500000357627869 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (4.699999988079071 : 0.07071065283054564 : Nil) & (0.15000000596046448 : 0.035355368562121334 : Nil) & (64.0 : 0.0 : Nil) & (0.8499999940395355 : 0.0 : Nil) & (0.75 : 0.0 : Nil) & (0.9000000059604645 : 0.0 : Nil) & (1.699999988079071 : 0.1414213478079398 : Nil) \\
pattern-match & (0.050000011920928955 : 0.03535534748869708 : Nil) & (2.1500000059604645 : 0.03535532641527282 : Nil) & (0.0 : 0.0 : Nil) & (2.850000023841858 : 0.10606600031924272 : Nil) & (0.6499999761581421 : 0.03535534748869708 : Nil) & (52.5 : 0.0 : Nil) & (0.5999999940395355 : 0.0707106739039699 : Nil) & (0.45000001788139343 : 0.03535532641527282 : Nil) & (0.7499999701976776 : 0.03535532641527282 : Nil) & (0.7000000178813934 : 2.1073424255447014e-8 : Nil) \\
range & (0.20000001788139343 : 2.1073424255447014e-8 : Nil) & (2.699999988079071 : 0.1414213478079398 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (7.199999988079071 : 0.21213204278533396 : Nil) & (0.4000000059604645 : 2.1073424255447014e-8 : Nil) & (105.0 : 0.0 : Nil) & (2.3499999940395355 : 0.03535532641527282 : Nil) & (2.6500000059604645 : 0.10606602139266698 : Nil) & (2.5 : 0.1414213478079398 : Nil) & (1.25 : 0.0 : Nil) \\
records & (0.1499999761581421 : 0.03535534748869708 : Nil) & (1.9000000059604645 : 2.1073424255447014e-8 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (3.0499999821186066 : 0.17677671637006112 : Nil) & (0.550000011920929 : 0.03535534748869708 : Nil) & (57.5 : 0.0 : Nil) & (0.5999999940395355 : 2.1073424255447014e-8 : Nil) & (0.8500000238418579 : 0.10606600031924272 : Nil) & (0.7500000298023224 : 0.03535532641527282 : Nil) & (0.7000000178813934 : 2.1073424255447014e-8 : Nil) \\
record-lookup & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (0.0 : 0.0 : Nil) & (0.550000011920929 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 0.0707106739039699 : Nil) & (14.5 : 0.0 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (0.25 : 0.03535530534184857 : Nil) & (0.09999999403953552 : 0.0 : Nil) \\
reverse & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.3500000238418579 : 0.03535534748869708 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.8499999642372131 : 0.03535534748869708 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (16.5 : 0.0 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.20000001788139343 : 2.1073424255447014e-8 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (0.25 : 0.03535534748869708 : Nil) \\
slicing/add & (0.09999999403953552 : 0.0707106739039699 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.20000001788139343 : 2.1073424255447014e-8 : Nil) & (0.20000001788139343 : 0.0707106739039699 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (5.5 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.0 : 0.0 : Nil) \\
slicing/array/lookup & (0.09999999403953552 : 0.0 : Nil) & (5.0999999940395355 : 0.0707106739039699 : Nil) & (0.25 : 0.10606600031924272 : Nil) & (12.0 : 0.07071069497739416 : Nil) & (0.3999999761581421 : 0.07071069497739416 : Nil) & (210.0 : 0.0 : Nil) & (3.9000000059604645 : 0.28284271668930383 : Nil) & (3.7999999821186066 : 0.3535533695198495 : Nil) & (4.0 : 0.1414213478079398 : Nil) & (1.9000000059604645 : 0.0 : Nil) \\
slicing/array/dims & (0.20000001788139343 : 0.0707106739039699 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.4999999701976776 : 0.0707106739039699 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (12.0 : 0.0 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) \\
slicing/convolution/edge-detect & (129.80000001192093 : 0.4242640434238194 : Nil) & (321.15000000596046 : 3.4294678845400703 : Nil) & (6.549999982118607 : 0.24748736920060677 : Nil) & (1073.199999988079 : 10.960155108391486 : Nil) & (10.199999988079071 : 0.2828427377627281 : Nil) & (13522.5 : 0.0 : Nil) & (317.10000002384186 : 3.6769552537406773 : Nil) & (279.44999998807907 : 4.914392120817135 : Nil) & (331.10000002384186 : 6.222539682870988 : Nil) & (313.0499999821186 : 3.075914493946797 : Nil) \\
slicing/convolution/emboss & (117.89999997615814 : 0.7071067811865475 : Nil) & (244.10000002384186 : 6.717514421272201 : Nil) & (4.9000000059604645 : 0.2121320217119097 : Nil) & (877.2999999821186 : 13.222896820832492 : Nil) & (6.9000000059604645 : 0.14142132673451555 : Nil) & (10732.0 : 0.0 : Nil) & (272.75 : 3.783021296206768 : Nil) & (236.5 : 2.82842712474619 : Nil) & (277.85000002384186 : 5.550788249173137 : Nil) & (295.05000001192093 : 1.3081475620538523 : Nil) \\
slicing/convolution/gaussian & (134.9500000178814 : 9.652007567411058 : Nil) & (239.44999998807907 : 5.762920249811622 : Nil) & (4.25 : 0.24748739027403102 : Nil) & (858.1499999761581 : 13.541094842863645 : Nil) & (6.6500000059604645 : 0.10606602139266698 : Nil) & (10732.0 : 0.0 : Nil) & (268.35000002384186 : 0.31819804310457667 : Nil) & (236.80000001192093 : 2.5455844291303102 : Nil) & (287.59999999403954 : 12.232947301883216 : Nil) & (287.75 : 10.146982284738847 : Nil) \\
slicing/dict/create & (0.04999998211860657 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (7.5 : 0.0 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.0 : 0.0 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) \\
slicing/dict/difference & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.25 : 0.0 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (12.0 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) \\
slicing/dict/disjointUnion & (0.04999998211860657 : 0.0 : Nil) & (0.15000003576278687 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.3500000238418579 : 0.03535534748869708 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (9.5 : 0.0 : Nil) & (0.0 : 0.0 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.04999998211860657 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) \\
slicing/dict/foldl & (0.1499999761581421 : 0.03535534748869708 : Nil) & (1.2500000298023224 : 0.10606602139266698 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (3.5 : 0.35355339059327373 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (55.0 : 0.0 : Nil) & (1.050000011920929 : 0.03535534748869708 : Nil) & (1.5999999940395355 : 0.14142132673451555 : Nil) & (1.4000000059604645 : 0.0707106739039699 : Nil) & (1.2999999821186066 : 0.14142136888136406 : Nil) \\
slicing/dict/intersectionWith & (0.25 : 0.03535534748869708 : Nil) & (0.3499999940395355 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (1.0 : 0.2828426956158796 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (23.5 : 0.0 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.4000000059604645 : 2.1073424255447014e-8 : Nil) & (0.19999998807907104 : 0.07071069497739416 : Nil) & (0.15000003576278687 : 0.03535534748869708 : Nil) \\
slicing/dict/fromRecord & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.19999998807907104 : 0.07071065283054564 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (5.0 : 0.0 : Nil) & (0.0 : 0.0 : Nil) & (0.10000002384185791 : 0.07071069497739416 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.0 : 0.0 : Nil) \\
slicing/dict/get & (0.050000011920928955 : 0.0 : Nil) & (0.3499999940395355 : 0.10606602139266698 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.6500000059604645 : 0.24748736920060677 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (14.5 : 0.0 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) \\
slicing/dict/map & (0.09999999403953552 : 0.0 : Nil) & (0.800000011920929 : 0.07071069497739416 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (1.3000000417232513 : 0.0707106739039699 : Nil) & (0.29999998211860657 : 2.1073424255447014e-8 : Nil) & (35.5 : 0.0 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (0.699999988079071 : 0.1414213478079398 : Nil) & (0.2499999701976776 : 0.10606602139266698 : Nil) & (0.15000000596046448 : 0.0 : Nil) \\
slicing/divide & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.20000001788139343 : 0.0707106739039699 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (3.5 : 0.0 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.04999998211860657 : 0.0 : Nil) & (0.0 : 0.0 : Nil) \\
slicing/dtw/compute-dtw & (5501.549999982119 : 21.177848109181152 : Nil) & (74.94999998807907 : 1.0960155192685184 : Nil) & (5.899999976158142 : 0.21213204278533396 : Nil) & (214.7000000178814 : 3.111269841435494 : Nil) & (24.650000005960464 : 0.6717514547712746 : Nil) & (3006.5 : 0.0 : Nil) & (62.849999994039536 : 1.5202795837657619 : Nil) & (74.10000002384186 : 3.0405591675315238 : Nil) & (70.84999999403954 : 3.5001785795174647 : Nil) & (62.04999998211861 : 1.2374368881498823 : Nil) \\
slicing/dtw/average-series & (4898.800000011921 : 99.06566006109404 : Nil) & (110.39999997615814 : 0.49497473840121353 : Nil) & (1.6500000059604645 : 0.10606602139266698 : Nil) & (239.04999995231628 : 2.651650429449553 : Nil) & (15.550000011920929 : 0.10606604246609123 : Nil) & (3272.0 : 0.0 : Nil) & (72.14999997615814 : 1.661700952647126 : Nil) & (79.75000002980232 : 0.8131728025792144 : Nil) & (80.55000001192093 : 1.0960155192685184 : Nil) & (73.80000001192093 : 0.21213204278533396 : Nil) \\
slicing/filter & (0.5999999940395355 : 0.0707106739039699 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (1.6500000059604645 : 0.10606602139266698 : Nil) & (0.3499999940395355 : 0.03535532641527282 : Nil) & (27.0 : 0.0 : Nil) & (0.5 : 0.1414213478079398 : Nil) & (0.3499999940395355 : 0.03535532641527282 : Nil) & (0.7000000178813934 : 0.14142136888136406 : Nil) & (0.6500000059604645 : 0.10606602139266698 : Nil) \\
slicing/intersperse & (0.25 : 0.0 : Nil) & (0.3499999940395355 : 0.035355368562121334 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (1.2500000298023224 : 0.10606602139266698 : Nil) & (0.6000000238418579 : 0.1414213478079398 : Nil) & (25.5 : 0.0 : Nil) & (0.550000011920929 : 0.17677669529663687 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.5499999523162842 : 0.17677669529663687 : Nil) & (0.25 : 0.03535534748869708 : Nil) \\
slicing/intersperse & (0.4000000059604645 : 2.1073424255447014e-8 : Nil) & (0.5999999940395355 : 0.14142136888136406 : Nil) & (0.44999998807907104 : 0.17677669529663687 : Nil) & (1.449999988079071 : 0.24748739027403102 : Nil) & (0.45000001788139343 : 0.03535532641527282 : Nil) & (25.5 : 0.0 : Nil) & (0.20000001788139343 : 2.1073424255447014e-8 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.3499999940395355 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) \\
slicing/length & (0.4999999701976776 : 0.0707106739039699 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.29999998211860657 : 2.1073424255447014e-8 : Nil) & (1.350000023841858 : 0.31819804310457667 : Nil) & (0.3500000238418579 : 0.03535534748869708 : Nil) & (24.0 : 0.0 : Nil) & (0.20000001788139343 : 0.0707106739039699 : Nil) & (0.2499999701976776 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (0.25 : 0.03535530534184857 : Nil) \\
slicing/list-comp & (1.7000000178813934 : 0.0707106739039699 : Nil) & (3.949999988079071 : 0.17677669529663687 : Nil) & (0.5999999940395355 : 0.0707106739039699 : Nil) & (15.300000011920929 : 0.9192388239718814 : Nil) & (1.5499999821186066 : 0.03535532641527282 : Nil) & (189.5 : 0.0 : Nil) & (4.600000023841858 : 0.1414213478079398 : Nil) & (4.149999976158142 : 0.03535534748869708 : Nil) & (5.399999976158142 : 0.1414213478079398 : Nil) & (4.900000035762787 : 0.21213204278533396 : Nil) \\
slicing/list-comp & (1.649999976158142 : 0.03535534748869708 : Nil) & (1.850000023841858 : 0.0 : Nil) & (0.3999999761581421 : 0.07071069497739416 : Nil) & (13.949999988079071 : 0.03535534748869708 : Nil) & (2.2500000298023224 : 0.3181980641780009 : Nil) & (189.5 : 0.0 : Nil) & (5.4000000059604645 : 0.2121320217119097 : Nil) & (4.050000011920929 : 0.10606600031924272 : Nil) & (4.9000000059604645 : 0.14142136888136406 : Nil) & (5.6500000059604645 : 0.7424621076018203 : Nil) \\
slicing/lookup & (0.3499999940395355 : 0.0 : Nil) & (0.949999988079071 : 0.03535534748869708 : Nil) & (0.45000001788139343 : 0.10606602139266698 : Nil) & (2.5499999821186066 : 0.03535532641527282 : Nil) & (0.6500000059604645 : 0.03535532641527282 : Nil) & (48.0 : 0.0 : Nil) & (0.5999999940395355 : 0.0707106739039699 : Nil) & (0.25 : 0.0 : Nil) & (0.550000011920929 : 0.03535534748869708 : Nil) & (0.75 : 0.10606604246609123 : Nil) \\
slicing/map & (0.4000000059604645 : 0.14142136888136406 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (0.7999999821186066 : 0.2121320217119097 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (14.5 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (0.45000001788139343 : 0.10606602139266698 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) \\
slicing/matrix-update & (0.3499999940395355 : 0.03535532641527282 : Nil) & (24.69999998807907 : 0.5656854333786077 : Nil) & (0.3499999940395355 : 0.035355368562121334 : Nil) & (51.74999997019768 : 0.9545941503871542 : Nil) & (1.699999988079071 : 0.1414213478079398 : Nil) & (777.0 : 0.0 : Nil) & (14.799999982118607 : 0.28284271668930383 : Nil) & (12.050000041723251 : 0.4596194119859407 : Nil) & (14.949999988079071 : 0.10606600031924272 : Nil) & (16.000000029802322 : 0.8485281500679115 : Nil) \\
slicing/multiply & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (0.15000000596046448 : 0.0 : Nil) & (0.04999998211860657 : 0.0 : Nil) & (5.5 : 0.0 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.0 : 0.0 : Nil) & (0.0 : 0.0 : Nil) \\
slicing/nth & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.75 : 0.10606600031924272 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) & (1.2999999821186066 : 0.0707106739039699 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (19.0 : 0.0 : Nil) & (0.3999999761581421 : 0.07071069497739416 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.44999998807907104 : 0.10606600031924272 : Nil) & (0.25 : 0.03535534748869708 : Nil) \\
slicing/output-not-source & (0.050000011920928955 : 0.03535534748869708 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.1499999761581421 : 0.03535534748869708 : Nil) & (0.19999998807907104 : 0.07071069497739416 : Nil) & (0.04999998211860657 : 0.0 : Nil) & (4.5 : 0.0 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.050000011920928955 : 0.03535534748869708 : Nil) \\
slicing/section-5-example & (2.75 : 0.17677669529663687 : Nil) & (3.9500000178813934 : 0.03535532641527282 : Nil) & (0.25 : 0.0 : Nil) & (18.80000001192093 : 1.0606601717798212 : Nil) & (2.050000011920929 : 0.17677669529663687 : Nil) & (210.5 : 0.0 : Nil) & (5.6500000059604645 : 0.24748736920060677 : Nil) & (6.450000017881393 : 0.24748736920060677 : Nil) & (6.4000000059604645 : 0.6363961072825776 : Nil) & (6.299999982118607 : 2.1073424255447014e-8 : Nil) \\
slicing/section-5-example & (1.6500000059604645 : 0.1767766742232126 : Nil) & (4.700000017881393 : 0.0707106739039699 : Nil) & (0.1499999761581421 : 0.0 : Nil) & (15.599999994039536 : 0.0707106739039699 : Nil) & (1.300000011920929 : 0.07071069497739416 : Nil) & (210.5 : 0.0 : Nil) & (5.200000017881393 : 0.0707106739039699 : Nil) & (2.75 : 0.0 : Nil) & (5.399999976158142 : 0.07071069497739416 : Nil) & (5.75 : 0.17677669529663687 : Nil) \\
slicing/section-5-example & (0.9000000059604645 : 0.0 : Nil) & (4.3499999940395355 : 0.24748736920060677 : Nil) & (0.3499999940395355 : 0.03535532641527282 : Nil) & (14.599999964237213 : 0.1414213478079398 : Nil) & (0.75 : 0.0 : Nil) & (210.5 : 0.0 : Nil) & (5.1500000059604645 : 0.3181980641780009 : Nil) & (5.300000011920929 : 0.49497473840121353 : Nil) & (5.150000035762787 : 0.03535534748869708 : Nil) & (5.300000011920929 : 0.1414213478079398 : Nil) \\
slicing/zeros & (0.3500000238418579 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 0.0707106739039699 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.3500000238418579 : 0.03535534748869708 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (11.5 : 0.0 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.09999999403953552 : 0.0 : Nil) & (0.15000003576278687 : 0.03535534748869708 : Nil) \\
slicing/zeros & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.15000000596046448 : 0.03535532641527282 : Nil) & (0.050000011920928955 : 0.0 : Nil) & (0.45000001788139343 : 0.03535532641527282 : Nil) & (0.20000001788139343 : 2.1073424255447014e-8 : Nil) & (11.5 : 0.0 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (0.04999998211860657 : 0.03535532641527282 : Nil) & (0.2499999701976776 : 0.10606602139266698 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) \\
slicing/zipWith & (0.5999999940395355 : 2.1073424255447014e-8 : Nil) & (0.4000000059604645 : 0.0 : Nil) & (0.15000000596046448 : 0.035355368562121334 : Nil) & (2.350000023841858 : 0.03535534748869708 : Nil) & (0.5499999821186066 : 0.03535532641527282 : Nil) & (48.5 : 0.0 : Nil) & (0.5 : 0.07071069497739416 : Nil) & (0.25 : 0.0 : Nil) & (0.5999999940395355 : 0.14142136888136406 : Nil) & (0.5999999940395355 : 0.0707106739039699 : Nil) \\
slicing/linked-outputs/bar-chart-line-chart & (20.849999994039536 : 1.7324116265510958 : Nil) & (2525.0500000417233 : 27.824651835475958 : Nil) & (26.25 : 1.7324116054776717 : Nil) & (4515.999999970198 : 1105.0664776256924 : Nil) & (176.15000000596046 : 0.10606602139266698 : Nil) & (27374.0 : 0.0 : Nil) & (2294.050000011921 : 38.28983218439281 : Nil) & (1258.6000000238419 : 107.12667734976195 : Nil) & (1894.8500000238419 : 559.9225046994263 : Nil) & (2366.050000011921 : 82.48400600855203 : Nil) \\
slicing/linked-outputs/stacked-bar-chart-scatter-plot & (98.14999997615814 : 24.996224731803192 : Nil) & (13063.050000011921 : 1189.8132253466854 : Nil) & (51.89999997615814 : 6.505382378486867 : Nil) & (11016.750000029802 : 3402.2089223526577 : Nil) & (7634.3499999940395 : 1207.6323162452304 : Nil) & (12494.5 : 0.0 : Nil) & (2557.0999999940395 : 21.56675684726312 : Nil) & (800.4499999582767 : 194.20687745709995 : Nil) & (1715.0999999940395 : 402.4144691690495 : Nil) & (3159.199999988079 : 99.41921345168731 : Nil) \\
graphics/background & (0.10000002384185791 : 0.07071069497739416 : Nil) & (1.699999988079071 : 0.07071069497739416 : Nil) & (0.09999999403953552 : 2.1073424255447014e-8 : Nil) & (2.25 : 0.17677669529663687 : Nil) & (0.20000001788139343 : 0.0 : Nil) & (45.5 : 0.0 : Nil) & (0.25 : 0.03535534748869708 : Nil) & (0.2500000298023224 : 0.03535532641527282 : Nil) & (0.3500000238418579 : 0.03535534748869708 : Nil) & (0.25 : 0.03535534748869708 : Nil) \\
graphics/grouped-bar-chart & (2.9500000178813934 : 0.10606602139266698 : Nil) & (1053.0499999821186 : 3.7830212751333443 : Nil) & (0.5 : 0.0 : Nil) & (675.3499999940395 : 4.560838751297286 : Nil) & (516.7499999701977 : 0.9545941503871542 : Nil) & (1492.5 : 0.0 : Nil) & (37.45000001788139 : 0.4596194119859407 : Nil) & (38.44999998807907 : 0.17677669529663687 : Nil) & (45.599999994039536 : 0.0707106739039699 : Nil) & (37.75 : 0.10606600031924272 : Nil) \\
graphics/line-chart & (1.5999999940395355 : 2.1073424255447014e-8 : Nil) & (432.55000001192093 : 0.03535534748869708 : Nil) & (1.600000023841858 : 0.07071069497739416 : Nil) & (535.9500000178814 : 4.419417403489346 : Nil) & (187.25 : 0.9545941714605785 : Nil) & (2179.5 : 0.0 : Nil) & (48.30000001192093 : 0.7071067811865475 : Nil) & (54.45000001788139 : 1.1667261931724882 : Nil) & (56.19999998807907 : 4.171929992141891 : Nil) & (58.400000005960464 : 0.49497475947463776 : Nil) \\
graphics/stacked-bar-chart & (2.0499999821186066 : 0.10606602139266698 : Nil) & (609.8000000119209 : 3.0405591675315238 : Nil) & (0.75 : 0.03535530534184857 : Nil) & (389.4500000178814 : 6.540737747048988 : Nil) & (286.94999998807907 : 1.0253048242911242 : Nil) & (1022.5 : 0.0 : Nil) & (10.699999988079071 : 0.0 : Nil) & (23.349999994039536 : 0.10606602139266698 : Nil) & (23.599999964237213 : 1.6263456051584289 : Nil) & (22.399999976158142 : 0.4242640855706679 : Nil) \\
\bottomrule
\end{tabular}
\end{table}


==> fig/performance/demands-speedup.tex <==
\begin{longtable}{lrrr}
\caption{Demands Times Traces Versus Graphs} \label{table:demands-speedups} \\
\toprule
 & \textbf{T-Demands} & \textbf{G-Demands} & \textbf{Bwd-Speedup} \\
\midrule
\endfirsthead
\caption[]{Demands Times Traces Versus Graphs} \\
\toprule
 & \textbf{T-Demands} & \textbf{G-Demands} & \textbf{Bwd-Speedup} \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
\textbf{compute-dtw} & 76.23 & 5.97 & 12.78 \\
\textbf{edge-detect} & 279.03 & 5.53 & 50.43 \\
\textbf{emboss} & 234.77 & 3.67 & 64.03 \\
\textbf{gaussian} & 230.30 & 7.27 & 31.69 \\
\textbf{bar-chart-line-chart} & 544.03 & 11.40 & 47.72 \\
\textbf{stacked-bar-chart-scatter-plot} & 406.80 & 8.43 & 48.24 \\
\textbf{grouped-bar-chart} & 107.07 & 2.17 & 49.42 \\
\textbf{line-chart} & 158.23 & 4.07 & 38.91 \\
\textbf{stacked-bar-chart} & 70.97 & 3.67 & 19.35 \\
\end{longtable}


==> fig/performance/eval-speedup.tex <==
\begin{longtable}{lrrr}
\caption{Evaluation Time of Traces Versus Graphs (ms)} \label{table:eval-speedups} \\
\toprule
 & T-Eval & G-Eval & Eval-Speedup \\
\midrule
\endfirsthead
\caption[]{Evaluation Time of Traces Versus Graphs (ms)} \\
\toprule
 & T-Eval & G-Eval & Eval-Speedup \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
compute-dtw & 77.23 & 225.23 & 0.34 \\
edge-detect & 346.23 & 1063.53 & 0.33 \\
emboss & 313.10 & 846.77 & 0.37 \\
gaussian & 280.37 & 849.67 & 0.33 \\
bar-chart-line-chart & 1085.90 & 2897.13 & 0.37 \\
stacked-bar-chart-scatter-plot & 1049.20 & 6698.30 & 0.16 \\
grouped-bar-chart & 128.77 & 1933.23 & 0.07 \\
line-chart & 192.07 & 1845.70 & 0.10 \\
stacked-bar-chart & 81.67 & 1255.93 & 0.07 \\
\end{longtable}


==> fig/performance/expensive-bwd.tex <==
\begin{table}
\caption{Tests: expensive, Benches: bwd}
\label{expensive-bwd}
\begin{tabular}{lrrrr}
\toprule
 & T-Eval & T-Bwd & G-Eval & G-Bwd \\
Test-Name &  &  &  &  \\
\midrule
slicing/convolution/edge-detect & 741.00 & 503.50 & 1290.20 & 5.00 \\
slicing/convolution/emboss & 626.80 & 409.60 & 1084.50 & 4.50 \\
slicing/convolution/gaussian & 647.90 & 415.10 & 1098.40 & 4.00 \\
graphics/grouped-bar-chart & 83.70 & 64.10 & 134.10 & 1.50 \\
graphics/line-chart & 142.30 & 96.50 & 232.20 & 2.20 \\
graphics/stacked-bar-chart & 47.00 & 38.00 & 97.80 & 1.50 \\
slicing/dtw/compute-dtw & 163.10 & 133.90 & 317.70 & 19.60 \\
\bottomrule
\end{tabular}
\end{table}


==> fig/performance/expensive-fwd.tex <==
\begin{table}
\caption{Tests: expensive, Benches: fwd}
\label{expensive-fwd}
\begin{tabular}{lrrrrr}
\toprule
 & T-Eval & T-Fwd & G-Eval & G-Fwd & Naive-Fwd \\
Test-Name &  &  &  &  &  \\
\midrule
slicing/convolution/edge-detect & 741.00 & 638.40 & 1290.20 & 3.70 & 2097.40 \\
slicing/convolution/emboss & 626.80 & 567.40 & 1084.50 & 1.40 & 1945.70 \\
slicing/convolution/gaussian & 647.90 & 569.10 & 1098.40 & 1.80 & 1934.50 \\
graphics/grouped-bar-chart & 83.70 & 79.30 & 134.10 & 147.30 & 1862.40 \\
graphics/line-chart & 142.30 & 111.10 & 232.20 & 672.50 & 3157.40 \\
graphics/stacked-bar-chart & 47.00 & 46.10 & 97.80 & 98.10 & 126.70 \\
slicing/dtw/compute-dtw & 163.10 & 194.10 & 317.70 & 17.70 & 176.90 \\
\bottomrule
\end{tabular}
\end{table}


==> fig/performance/slicing-speedup.tex <==
  \DOnote{Missing units in the columns here. I assume T-Fwd, G-Fwd, T-Bwd, and G-Bwd are secods but should be stated.}
\begin{longtable}{lrrrrrr}
\caption{Slicing times and average speedups} \label{table:slicing-speedups} \\
\toprule
 & T-Fwd & G-Fwd & Fwd-Speedup & T-Bwd & G-Bwd & Bwd-Speedup \\
Test-Name &  &  &  &  &  &  \\
\midrule
\endfirsthead
\caption[]{Slicing times and average speedups} \\
\toprule
 & T-Fwd & G-Fwd & Fwd-Speedup & T-Bwd & G-Bwd & Bwd-Speedup \\
Test-Name &  &  &  &  &  &  \\
\midrule
\endhead
\midrule
\multicolumn{7}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
arithmetic & 0.30 & 0.02 & 15.17 & 2.37 & 0.23 & 10.32 \\
array & 1.03 & 0.05 & 22.14 & 2.76 & 0.26 & 10.62 \\
compose & 0.21 & 0.01 & 15.50 & 2.26 & 0.23 & 9.97 \\
dicts & 0.39 & 0.27 & 1.43 & 2.61 & 0.21 & 12.41 \\
div-mod-quot-rem & 0.52 & 0.84 & 0.62 & 2.49 & 0.31 & 8.04 \\
factorial & 1.96 & 0.01 & 196.33 & 3.06 & 0.23 & 13.30 \\
filter & 1.08 & 0.03 & 32.30 & 2.67 & 0.20 & 13.56 \\
first-class-constr & 0.82 & 0.08 & 10.29 & 2.40 & 0.24 & 9.99 \\
flatten & 1.88 & 0.12 & 16.09 & 2.89 & 0.23 & 12.39 \\
foldr-sumSquares & 1.38 & 0.01 & 138.33 & 2.82 & 0.21 & 13.65 \\
lexicalScoping & 0.35 & 0.01 & 26.00 & 2.57 & 0.24 & 10.55 \\
length & 0.38 & 0.01 & 37.67 & 2.37 & 0.21 & 11.12 \\
lookup & 1.70 & 0.02 & 72.71 & 3.08 & 0.27 & 11.54 \\
map & 1.43 & 0.11 & 13.41 & 3.33 & 0.28 & 12.02 \\
mergeSort & 5.98 & 0.04 & 149.58 & 4.26 & 0.20 & 21.28 \\
normalise & 0.33 & 0.02 & 14.00 & 2.43 & 0.21 & 11.38 \\
pattern-match & 1.85 & 0.01 & 184.67 & 2.61 & 0.23 & 11.53 \\
range & 5.82 & 0.11 & 54.59 & 6.24 & 0.22 & 28.82 \\
records & 2.06 & 0.04 & 51.50 & 3.31 & 0.23 & 14.39 \\
reverse & 0.71 & 0.03 & 23.67 & 2.39 & 0.23 & 10.23 \\
desugar/list-comp-1 & 7.74 & 0.13 & 59.54 & 8.03 & 0.25 & 31.71 \\
desugar/list-comp-2 & 22.73 & 0.95 & 24.01 & 19.87 & 0.28 & 70.12 \\
desugar/list-comp-3 & 6.05 & 0.03 & 181.40 & 7.16 & 0.21 & 33.58 \\
desugar/list-comp-4 & 3.00 & 0.03 & 90.00 & 3.89 & 0.23 & 16.66 \\
desugar/list-comp-5 & 1.96 & 0.04 & 45.31 & 3.36 & 0.24 & 13.82 \\
desugar/list-comp-6 & 0.10 & 0.02 & 6.20 & 2.13 & 0.26 & 8.31 \\
desugar/list-comp-7 & 2.29 & 0.02 & 137.40 & 3.21 & 0.21 & 15.03 \\
desugar/list-enum & 1.36 & 0.07 & 20.45 & 2.99 & 0.19 & 16.04 \\
slicing/add & 0.05 & 0.14 & 0.39 & 2.31 & 0.39 & 5.92 \\
slicing/array/lookup & 10.70 & 0.05 & 214.07 & 10.10 & 0.35 & 29.13 \\
slicing/array/dims & 0.85 & 0.30 & 2.87 & 2.80 & 0.45 & 6.28 \\
slicing/convolution/edge-detect & 690.69 & 4.22 & 163.80 & 509.97 & 5.87 & 86.93 \\
slicing/convolution/emboss & 611.36 & 1.85 & 329.87 & 420.70 & 4.25 & 98.91 \\
slicing/convolution/gaussian & 560.75 & 1.71 & 327.92 & 389.42 & 3.82 & 102.03 \\
slicing/dict/create & 0.04 & 0.06 & 0.61 & 2.18 & 0.31 & 7.11 \\
slicing/dict/difference & 0.29 & 0.07 & 4.40 & 2.26 & 0.26 & 8.82 \\
slicing/dict/disjointUnion & 0.13 & 0.11 & 1.19 & 2.52 & 0.38 & 6.58 \\
slicing/dict/foldl & 2.48 & 0.07 & 35.38 & 4.24 & 0.28 & 15.34 \\
slicing/dict/intersectionWith & 0.39 & 0.15 & 2.57 & 2.53 & 0.37 & 6.85 \\
slicing/dict/fromRecord & 0.07 & 0.11 & 0.69 & 2.28 & 0.30 & 7.70 \\
slicing/dict/get & 0.22 & 0.05 & 4.33 & 2.37 & 0.29 & 8.09 \\
slicing/dict/map & 0.78 & 0.11 & 7.28 & 2.88 & 0.39 & 7.45 \\
slicing/divide & 0.02 & 0.08 & 0.22 & 2.14 & 0.32 & 6.61 \\
slicing/filter & 1.38 & 0.29 & 4.72 & 2.83 & 0.33 & 8.48 \\
slicing/intersperse & 0.93 & 0.21 & 4.36 & 2.28 & 0.29 & 7.77 \\
slicing/intersperse & 0.83 & 0.33 & 2.51 & 2.38 & 0.38 & 6.33 \\
slicing/length & 0.77 & 0.29 & 2.66 & 2.39 & 0.58 & 4.14 \\
slicing/list-comp & 10.94 & 0.98 & 11.12 & 9.47 & 0.47 & 20.29 \\
slicing/list-comp & 10.80 & 0.93 & 11.66 & 9.89 & 0.40 & 24.51 \\
slicing/lookup & 1.51 & 0.46 & 3.28 & 3.23 & 0.46 & 6.98 \\
slicing/map & 0.45 & 0.18 & 2.47 & 2.49 & 0.27 & 9.12 \\
slicing/multiply & 0.05 & 0.06 & 0.79 & 2.22 & 0.30 & 7.49 \\
slicing/nth & 0.75 & 0.04 & 17.31 & 2.55 & 0.35 & 7.29 \\
slicing/section-5-example & 11.17 & 1.04 & 10.71 & 10.44 & 0.46 & 22.86 \\
slicing/section-5-example & 10.08 & 0.41 & 24.80 & 9.98 & 0.36 & 27.47 \\
slicing/section-5-example & 11.32 & 0.58 & 19.41 & 11.00 & 0.42 & 26.40 \\
slicing/zeros & 0.47 & 0.27 & 1.78 & 2.27 & 0.37 & 6.09 \\
slicing/zeros & 0.51 & 0.18 & 2.91 & 2.61 & 0.47 & 5.52 \\
slicing/zipWith & 1.90 & 0.40 & 4.71 & 2.94 & 0.38 & 7.68 \\
slicing/matrix-update & 30.37 & 0.34 & 89.31 & 23.65 & 0.38 & 62.24 \\
slicing/dtw/compute-dtw & 117.31 & 14.09 & 8.33 & 109.24 & 2.67 & 40.97 \\
graphics/background & 0.73 & 0.70 & 1.04 & 2.59 & 0.85 & 3.06 \\
graphics/grouped-bar-chart & 70.74 & 125.64 & 0.56 & 59.25 & 1.29 & 45.81 \\
graphics/line-chart & 101.03 & 409.60 & 0.25 & 86.63 & 1.24 & 69.68 \\
graphics/stacked-bar-chart & 36.67 & 74.08 & 0.49 & 32.63 & 1.03 & 31.68 \\
\end{longtable}


==> tex-common/MnSymbol-asterisk.tex <==
% Bring in asterisk symbols from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\Mnthinstar}{\mathrel}{MnSyC}{134}
\DeclareMathSymbol{\Mnast}{\mathrel}{MnSyC}{135}


==> tex-common/MnSymbol-bowtie.tex <==
\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\let\bowtie\relax
\DeclareMathSymbol{\bowtie}{\mathrel}{MnSyC}{38}


==> tex-common/MnSymbol-cong.tex <==
% Bring in \cong from MnSymbol.

\DeclareFontFamily{U}{MnSymbolD}{}
\DeclareFontShape{U}{MnSymbolD}{m}{n}{
    <-6>  MnSymbolD5
   <6-7>  MnSymbolD6
   <7-8>  MnSymbolD7
   <8-9>  MnSymbolD8
   <9-10> MnSymbolD9
  <10-12> MnSymbolD10
  <12->   MnSymbolD12}{}
\DeclareFontShape{U}{MnSymbolD}{b}{n}{
    <-6>  MnSymbolD-Bold5
   <6-7>  MnSymbolD-Bold6
   <7-8>  MnSymbolD-Bold7
   <8-9>  MnSymbolD-Bold8
   <9-10> MnSymbolD-Bold9
  <10-12> MnSymbolD-Bold10
  <12->   MnSymbolD-Bold12}{}
\DeclareSymbolFont{MnSyD}{U}{MnSymbolD}{m}{n}

\DeclareMathSymbol{\Cong}{\mathrel}{MnSyD}{12}


==> tex-common/MnSymbol-inequalities.tex <==
\DeclareFontFamily{U}{MnSymbolD}{}
\DeclareFontShape{U}{MnSymbolD}{m}{n}{
    <-6>  MnSymbolD5
   <6-7>  MnSymbolD6
   <7-8>  MnSymbolD7
   <8-9>  MnSymbolD8
   <9-10> MnSymbolD9
  <10-12> MnSymbolD10
  <12->   MnSymbolD12}{}
\DeclareFontShape{U}{MnSymbolD}{b}{n}{
    <-6>  MnSymbolD-Bold5
   <6-7>  MnSymbolD-Bold6
   <7-8>  MnSymbolD-Bold7
   <8-9>  MnSymbolD-Bold8
   <9-10> MnSymbolD-Bold9
  <10-12> MnSymbolD-Bold10
  <12->   MnSymbolD-Bold12}{}
\DeclareSymbolFont{MnSyD}{U}{MnSymbolD}{m}{n}

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\sqcupdot}{\mathrel}{MnSyC}{68}
\DeclareMathSymbol{\sqcapdot}{\mathrel}{MnSyC}{69}
\DeclareMathSymbol{\eqslantgtr}{\mathrel}{MnSyC}{228}
\DeclareMathSymbol{\eqslantless}{\mathrel}{MnSyC}{227}

\DeclareMathSymbol{\less}{\mathrel}{MnSyD}{64}
\DeclareMathSymbol{\gtr}{\mathrel}{MnSyD}{65}
\DeclareMathSymbol{\leqslant}{\mathrel}{MnSyD}{68}
\DeclareMathSymbol{\geqslant}{\mathrel}{MnSyD}{69}
\DeclareMathSymbol{\sqlt}{\mathrel}{MnSyD}{88}
\DeclareMathSymbol{\sqgt}{\mathrel}{MnSyD}{89}
\DeclareMathSymbol{\sqleq}{\mathrel}{MnSyD}{90}
\DeclareMathSymbol{\sqgeq}{\mathrel}{MnSyD}{91}
\DeclareMathSymbol{\lessdot}{\mathrel}{MnSyD}{114}
\DeclareMathSymbol{\greaterdot}{\mathrel}{MnSyD}{115}
\DeclareMathSymbol{\leqslantdot}{\mathrel}{MnSyD}{118}
\DeclareMathSymbol{\geqslantdot}{\mathrel}{MnSyD}{119}
\DeclareMathSymbol{\leqslant}{\mathrel}{MnSyD}{68}
\DeclareMathSymbol{\geqslant}{\mathrel}{MnSyD}{69}
\DeclareMathSymbol{\nsqleq}{\mathrel}{MnSyD}{210}
\DeclareMathSymbol{\nsqgeq}{\mathrel}{MnSyD}{211}


==> tex-common/MnSymbol-medsquare.tex <==
% Bring in \medsquare from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\medsquare}{\mathord}{MnSyC}{106}


==> tex-common/MnSymbol-powerset.tex <==
% Bring in \powerset from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\MnSymbolpowerset}{\mathord}{MnSyC}{180}


==> tex-common/MnSymbol-triangles.tex <==
% Various triangles from MnSymbol. See http://tex.stackexchange.com/questions/36006.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\smalltriangleright}{\mathord}{MnSyC}{72}
\DeclareMathSymbol{\smalltriangleup}{\mathord}{MnSyC}{73}
\DeclareMathSymbol{\smalltriangleleft}{\mathord}{MnSyC}{74}
\DeclareMathSymbol{\smalltriangledown}{\mathord}{MnSyC}{75}
\DeclareMathSymbol{\filledtriangleright}{\mathord}{MnSyC}{76}
\DeclareMathSymbol{\filledtriangleup}{\mathord}{MnSyC}{77}
\DeclareMathSymbol{\filledtriangleleft}{\mathord}{MnSyC}{78}
\DeclareMathSymbol{\filledtriangledown}{\mathord}{MnSyC}{79}


==> tex-common/MnSymbol-twoheadarrows.tex <==
\DeclareFontFamily{U}{MnSymbolB}{}
\DeclareFontShape{U}{MnSymbolB}{m}{n}{
    <-6>  MnSymbolB5
   <6-7>  MnSymbolB6
   <7-8>  MnSymbolB7
   <8-9>  MnSymbolB8
   <9-10> MnSymbolB9
  <10-12> MnSymbolB10
  <12->   MnSymbolB12}{}
\DeclareFontShape{U}{MnSymbolB}{b}{n}{
    <-6>  MnSymbolB-Bold5
   <6-7>  MnSymbolB-Bold6
   <7-8>  MnSymbolB-Bold7
   <8-9>  MnSymbolB-Bold8
   <9-10> MnSymbolB-Bold9
  <10-12> MnSymbolB-Bold10
  <12->   MnSymbolB-Bold12}{}
\DeclareSymbolFont{MnSyB}{U}{MnSymbolB}{m}{n}

\DeclareFontFamily{U}{MnSymbolA}{}
\DeclareFontShape{U}{MnSymbolA}{m}{n}{
    <-6>  MnSymbolA5
   <6-7>  MnSymbolA6
   <7-8>  MnSymbolA7
   <8-9>  MnSymbolA8
   <9-10> MnSymbolA9
  <10-12> MnSymbolA10
  <12->   MnSymbolA12}{}
\DeclareFontShape{U}{MnSymbolA}{b}{n}{
    <-6>  MnSymbolA-Aold5
   <6-7>  MnSymbolA-Aold6
   <7-8>  MnSymbolA-Aold7
   <8-9>  MnSymbolA-Aold8
   <9-10> MnSymbolA-Aold9
  <10-12> MnSymbolA-Aold10
  <12->   MnSymbolA-Aold12}{}
\DeclareSymbolFont{MnSyA}{U}{MnSymbolA}{m}{n}

\let\twoheaddownarrow\relax
\DeclareMathSymbol{\twoheaddownarrow}{\mathrel}{MnSyA}{27}
\let\twoheaduparrow\relax
\DeclareMathSymbol{\twoheaduparrow}{\mathrel}{MnSyA}{25}

\let\ntwoheaddownarrow\relax
\DeclareMathSymbol{\ntwoheaddownarrow}{\mathrel}{MnSyB}{27}
\let\ntwoheaduparrow\relax
\DeclareMathSymbol{\ntwoheaduparrow}{\mathrel}{MnSyB}{25}


==> tex-common/MnSymbol-vdots.tex <==
% Bring in \medsquare from MnSymbol.

\DeclareFontFamily{U}{MnSymbolC}{}
\DeclareFontShape{U}{MnSymbolC}{m}{n}{
    <-6>  MnSymbolC5
   <6-7>  MnSymbolC6
   <7-8>  MnSymbolC7
   <8-9>  MnSymbolC8
   <9-10> MnSymbolC9
  <10-12> MnSymbolC10
  <12->   MnSymbolC12}{}
\DeclareFontShape{U}{MnSymbolC}{b}{n}{
    <-6>  MnSymbolC-Bold5
   <6-7>  MnSymbolC-Bold6
   <7-8>  MnSymbolC-Bold7
   <8-9>  MnSymbolC-Bold8
   <9-10> MnSymbolC-Bold9
  <10-12> MnSymbolC-Bold10
  <12->   MnSymbolC-Bold12}{}
\DeclareSymbolFont{MnSyC}{U}{MnSymbolC}{m}{n}

\DeclareMathSymbol{\MnSymbolvdots}{\mathord}{MnSyC}{6}


==> tex-common/bigcdot.tex <==
% http://tex.stackexchange.com/questions/235118
\makeatletter
\newcommand*\bigcdot{\mathpalette\bigcdot@{.7}}
\newcommand*\bigcdot@[2]{\mathbin{\vcenter{\hbox{\scalebox{#2}{$\m@th#1\bullet$}}}}}
\makeatother


==> tex-common/curvetie.tex <==
% https://tex.stackexchange.com/questions/371292
% other solution based on halloweenmath, which is no longer in my TeX distribution...

\RequirePackage{pict2e}

\makeatletter
\DeclareRobustCommand{\curvetie}{\mathbin{\mathpalette\arc@bow@tie\relax}}
\newcommand{\arc@bow@tie}[2]{%
  \vcenter{\hbox{%
    \sbox\z@{$\m@th#1\otimes$}%
    \sbox\tw@{$\m@th\mkern1mu$}%
    \setlength{\unitlength}{\wd\z@}%
    \linethickness{.4\wd\tw@}%
    \begin{picture}(1,1)
    \polyline(0.7878,0.7878)(0.2122,0.2122)
    \polyline(0.2122,0.7878)(0.7878,0.2122)
    \put(0.5,0.5){\arc[-46,46]{0.4}}
    \put(0.5,0.5){\arc[134,226]{0.4}}
    \end{picture}%
  }}%
}
\makeatother


==> tex-common/line-shift.tex <==
% shift left, shift right line styles.

\usetikzlibrary{decorations}
\pgfdeclaredecoration{simple line}{initial}{
  \state{initial}[width=\pgfdecoratedpathlength-1sp]{\pgfmoveto{\pgfpointorigin}}
  \state{final}{\pgflineto{\pgfpointorigin}}
}
\tikzset{
   shift left/.style={decorate,decoration={simple line,raise=#1}},
   shift right/.style={decorate,decoration={simple line,raise=-1*#1}},
}


==> tex-common/mathabx-barharpoons.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathb10
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\leftbarharpoon}        {3}{mathb}{"DC}
\DeclareMathSymbol{\rightbarharpoon}       {3}{mathb}{"DD}
\DeclareMathSymbol{\barleftharpoon}        {3}{mathb}{"DE}
\DeclareMathSymbol{\barrightharpoon}       {3}{mathb}{"DF}


==> tex-common/mathabx-bigoslash.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\bigoslash}{1}{mathx}{"CD}


==> tex-common/mathabx-bigotimes.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\bigotimes}{1}{mathx}{"C2}


==> tex-common/mathabx-primes.tex <==
% Setup the matha font (from mathabx.sty) -- because mathabx.sty incompatible with
% amsmath package.
\DeclareFontFamily{U}{matha}{\hyphenchar\font45}
\DeclareFontShape{U}{matha}{m}{n}{
      <5> <6> <7> <8> <9> <10> gen * matha
      <10.95> matha10 <12> <14.4> <17.28> <20.74> <24.88> matha12
      }{}
\DeclareSymbolFont{matha}{U}{matha}{m}{n}

% Define some characters from mathabx.dcl.
\DeclareMathSymbol{\twoPrime}{3}{matha}{"32}
\DeclareMathSymbol{\threePrime}{3}{matha}{"33}
\DeclareMathSymbol{\fourPrime}{3}{matha}{"34}


==> tex-common/mathabx-sqbullet.tex <==
% From mathabx.sty.
\DeclareFontFamily{U}{mathb}{\hyphenchar\font45}
\DeclareFontShape{U}{mathb}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathb10
      }{}
\DeclareSymbolFont{mathb}{U}{mathb}{m}{n}

% From mathabx.dcl.
\DeclareMathSymbol{\sqbullet}{1}{mathb}{"0D}


==> tex-common/mathabx-wideparen.tex <==
% https://tex.stackexchange.com/questions/69323

%% code from mathabx.sty and mathabx.dcl
\DeclareFontFamily{U}{mathx}{\hyphenchar\font45}
\DeclareFontShape{U}{mathx}{m}{n}{
      <5> <6> <7> <8> <9> <10>
      <10.95> <12> <14.4> <17.28> <20.74> <24.88>
      mathx10
      }{}
\DeclareSymbolFont{mathx}{U}{mathx}{m}{n}
\DeclareFontSubstitution{U}{mathx}{m}{n}
\DeclareMathAccent{\widecheck}{0}{mathx}{"71}
\DeclareMathAccent{\wideparen}{0}{mathx}{"75}


==> tex-common/proof-helpers.tex <==
\RequirePackage{adjustbox}

% http://tex.stackexchange.com/questions/44933
\newcounter{myequation}
\makeatletter
\@addtoreset{equation}{myequation}
\makeatother

% http://tex.stackexchange.com/questions/82535
\newenvironment{proofalign}{\par\nobreak\small\noindent\flalign}{\endflalign}

\newcommand*{\proseDescription}{\paragraph{Prose description.}}
\newcommand*{\paragraphCase}[1]{\paragraph{\uline{#1}}}

\newcommand*{\absurd}[1]{\Absurd{\uline{#1}}}
\newcommand*{\Absurd}[1]{\textcolor{red}{#1}}
\newcommand*{\contradiction}{\Absurd{\bot}}
\newcommand*{\qedLocal}{\text{\ding{234}}\;}

\setlength{\ULdepth}{0.25em}
\newcommand*{\interCaseZero}[1]{%
& \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interCaseOne}[1]{%
& \indent \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interCaseTwo}[1]{%
& \indent\indent \textbf{\emph{Case}}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseZero}[1]{%
& \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseOne}[1]{%
& \indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseTwo}[1]{%
& \indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseThree}[1]{%
& \indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseFour}[1]{%
& \indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseFive}[1]{%
& \indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseSix}[1]{%
& \indent\indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}
\newcommand*{\interSubcaseSeven}[1]{%
& \indent\indent\indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.& %
\\[0.25em]%
}

\newcommand*{\introCaseDerivationZero}[2]{%
& \textbf{\emph{Case}}\ %
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}

\newcommand*{\introCaseZero}[1]{%
& \textbf{\emph{Case}}\ \uline{#1}.\;%
}

\newcommand*{\introSubcaseZero}[1]{%
& \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseOne}[1]{%
& \indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseTwo}[1]{%
& \indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseThree}[1]{%
& \indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseFour}[1]{%
& \indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}
\newcommand*{\introSubcaseFive}[1]{%
& \indent\indent\indent\indent\indent \textbf{$\sqbullet$}\ \uline{#1}.\;%
}

% define \derivationWidth as a proportion of textwidth

\newcommand*{\caseDerivation}[2]{%
\textbf{\emph{Case}}\ %
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}
\newcommand*{\subcaseDerivation}[2]{%
\textbf{\emph{Subcase}}\ %
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}
\newcommand*{\derivation}[2]{%
\begin{adjustbox}{varwidth=#1}%
#2
\end{adjustbox}%
}


==> tex-common/relational-override.tex <==
% http://tex.stackexchange.com/questions/360021
\makeatletter
\DeclareRobustCommand{\reloverrideleft}{\mathrel{\mathpalette\rel@override\vartriangleleft}}
\DeclareRobustCommand{\reloverrideright}{\mathrel{\mathpalette\rel@override\vartriangleright}}

\newcommand{\rel@override}[2]{%
  \vphantom{#2}%
  \ooalign{$\m@th#1-$\cr$\m@th#1#2$}%
}
\makeatother


==> tex-common/secbreak.tex <==
\RequirePackage{fdsymbol}

\newcommand*{\secbreakchar}{\smblklozenge}
\newcommand*{\secbreak}{
\begin{center}%
   $\secbreakchar\;\secbreakchar\;\secbreakchar$%
\end{center}%
}


==> tex-common/theorem-envs.tex <==
% Not needed for llncs.sty or acmart.cls.
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{definition}{Definition}[subsection]
\newtheorem{remark}{Remark}[section]
\newtheorem{example}{Example}[section]

% http://tex.stackexchange.com/questions/43966
\makeatletter
\def\th@plain{%
  \thm@notefont{}% same as heading font
  \itshape % body font
}
\def\th@definition{%
  \thm@notefont{}% same as heading font
  \normalfont % body font
}
\makeatother


==> tex-common/tilde.tex <==
% https://tex.stackexchange.com/questions/9363/how-does-one-insert-a-backslash-or-a-tilde-into-latex
\newcommand*{\Tilde}{\raise.17ex\hbox{$\scriptstyle\sim$}}


==> tex-common/wavey.tex <==
% http://tex.stackexchange.com/questions/80378. This looks great, but unfortunately doesn't
% work properly with the Listings package; need to come up with an MWE and post a question.
\usepackage{xparse}
\usepackage{marginnote}
\usepackage{soul}
\usepackage{lipsum}
\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathmorphing}

\newlength\LineWidth
\newlength\Amplitude
\newlength\SegLength

\setlength\LineWidth{0.4pt}
\setlength\Amplitude{1pt}
\setlength\SegLength{5pt}

\definecolor{HLcolor}{RGB}{240,0,0}

% The following code contains a variation of the great code by Antal S-Z
% in his answer to http://tex.stackexchange.com/a/6029/3954
%in TeX.SX

\newcommand\tikzmark[1]{%
  \tikz[overlay,remember picture] \node (#1) {};}

\makeatletter
\newcommand{\highlight@DoHighlight}{
  \draw[HLcolor,line width=\LineWidth,decorate,decoration={zigzag,amplitude=\Amplitude,segment length=\SegLength}]  ($(begin highlight)+(0,-2pt)$) -- ($(end highlight)+(0,-2pt)$) ;
}

\newcommand{\highlight@BeginHighlight}{
  \coordinate (begin highlight) at (0,0) ;
}

\newcommand{\highlight@EndHighlight}{
  \coordinate (end highlight) at (0,0) ;
}

\newdimen\highlight@previous
\newdimen\highlight@current

\DeclareRobustCommand*\highlight[1][]{%
  \SOUL@setup
  %
  \def\SOUL@preamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@BeginHighlight
      \highlight@EndHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@postamble{%
    \begin{tikzpicture}[overlay, remember picture]
      \highlight@EndHighlight
      \highlight@DoHighlight
    \end{tikzpicture}%
  }%
  %
  \def\SOUL@everyhyphen{%
    \discretionary{%
      \SOUL@setkern\SOUL@hyphkern
      \SOUL@sethyphenchar
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everyexhyphen##1{%
    \SOUL@setkern\SOUL@hyphkern
    \hbox{##1}%
    \discretionary{%
      \tikz[overlay, remember picture] \highlight@EndHighlight ;%
    }{%
    }{%
      \SOUL@setkern\SOUL@charkern
    }%
  }%
  %
  \def\SOUL@everysyllable{%
    \begin{tikzpicture}[overlay, remember picture]
      \path let \p0 = (begin highlight), \p1 = (0,0) in \pgfextra
        \global\highlight@previous=\y0
        \global\highlight@current =\y1
      \endpgfextra (0,0) ;
      \ifdim\highlight@current < \highlight@previous
        \highlight@DoHighlight
        \highlight@BeginHighlight
      \fi
    \end{tikzpicture}%
    \the\SOUL@syllable
    \tikz[overlay, remember picture] \highlight@EndHighlight ;%
  }%
  \SOUL@
}
\makeatother

\DeclareDocumentCommand\Wavey{O{red}O{1pt}O{5pt}m}{%
  \colorlet{HLcolor}{#1}
  \setlength\Amplitude{#2}%
  \setlength\SegLength{#3}%
  \tikzmark{endquote}\tikzmark{beginquote}\highlight{#4}%
}


==> tex-common/xspace-emdash-fix.tex <==
% https://tex.stackexchange.com/questions/263271
\xspaceremoveexception{-}
\makeatletter
\renewcommand*\@xspace@hook{%
\ifx\@let@token-%
\expandafter\@xspace@dash@i
\fi
}
\def\@xspace@dash@i-{\futurelet\@let@token\@xspace@dash@ii}
\def\@xspace@dash@ii{%
\ifx\@let@token-%
\else
\unskip
\fi
-%
}
\makeatother

